Separation Logic with Linearly Compositional Inductive Predicates and Set Data Constraints

We identify difference-bound set constraints (DBS), an analogy of difference-bound arithmetic constraints for sets. DBS can express not only set constraints but also arithmetic constraints over set elements. We integrate DBS into separation logic with linearly compositional inductive predicates, obtaining a logic thereof where set data constraints of linear data structures can be specified. We show that the satisfiability of this logic is decidable. A crucial step of the decision procedure is to compute the transitive closure of DBS-definable set relations, to capture which we propose an extension of quantified set constraints with Presburger Arithmetic (RQSPA). The satisfiability of RQSPA is then shown to be decidable by harnessing advanced automata-theoretic techniques.

==> section4-2.tex <==
%!TEX root = sofsem18.tex
 
%
%Let us start with the examples: 
%\[
%\Delta_{\slseg}(S, S') =  S = S' \cup \{\inf(S)\} \wedge \inf(S) \le \inf(S').
%\]
%
%%\tl{remark: this is equivalent to $S'\subseteq S \wedge \inf(S) \le \inf(S') \wedge \sup(S)=\sup(S')$.}
%%
%By a simple observation, we have 
%\[
%TC[\Delta_\slseg](S, S') = S' \subseteq S \wedge \sup(S \setminus S') \le \inf(S').
%\]
%%
%Similarly, for
%\[
%\Delta_{\plseg}(S, S') = S= S' \cup \{\inf(S)\} \wedge \inf(S') = \inf(S)+1,
%\]
%%
%we have
%\[
%\begin{array}{l}
%TC[\Delta_\plseg](S, S') = (S = S') \vee \\
%\hspace{1cm} (\emptyset \subset S' \wedge S' \subset S \wedge  \forall x.\ (x \in S \setminus S' \leftrightarrow \inf(S) \le x \le \inf(S') - 1)).
%\end{array}
%\]
%%
%For
%\[
%\Delta_{\ldllseg}(S, S') = S= S' \cup \{\sup(S)\} \wedge \sup(S') = \sup(S)-1,
%\]
%%
%we have
%\[
%\begin{array}{l}
%TC[\Delta_\ldllseg](S, S') = (S = S') \vee \\
%%\hspace{1cm}  (S' = \emptyset \wedge \emptyset \subset S \wedge S = \intval(\inf(S), \sup(S))) \vee  \\
%\hspace{1cm} (\emptyset \subset S' \wedge S' \subset S \wedge  \forall x.\ (x \in S \setminus S' \leftrightarrow \sup(S')+1 \le x \le \sup(S))).
%\end{array}
%\]
%
%
%We can also consider more examples by adapting the aforementioned ones.
%Let
%\[
%\Delta'_{\slseg}(S, S') = S = S' \cup \{\inf(S)\} \wedge \inf(S)+2 \le \inf(S').
%\]
%%
%Then 
%\[
%\begin{array}{l}
%TC[\Delta'_\slseg](S, S') = (S = S') \vee \\
%(S' \subset S \wedge \forall x \in S \setminus S'.\ x +2 \le \inf(S') \wedge \forall x, y \in S \setminus S'.\ x < y \rightarrow x+2 \le y).
%\end{array}
%\]
%\tl{here, disjunction is use!}
%\smallskip
%
%The formulae $TC[\Delta'_\slseg](S, S')$ belongs to the theory $\dbs$ defined in the previous section.
%
%We can also consider more examples by adapting the aforementioned ones.
%Let
%\[
%\Delta'_{\slseg}(S, S') = S = S' \cup \{\inf(S)\} \wedge \inf(S)+2 \le \inf(S').
%\]
%%

%=========================================
 

As we will see later, since $\lcslidset[P]$ involve inductive predicates, deciding its decidability requires, among others, the computation of transitive closure of difference-bound set relations which are defined by a $\dbs$ formula $\varphi(\vec{S}, \vec{S}')$. This is the main purpose of this subsection. We start with the special case $\varphi_R(S, S')$, where there is only one source/destination set parameter.
%
%\[
%\begin{array}{r c l c r}
%\varphi &::=& S\ \opset\ S' \cup T_s \mid  T_i \ \op\ T_i + c \mid \varphi \wedge \varphi & \\
%T_s & ::= & \emptyset \mid \{\min(S)\} \mid \{\max(S)\}\mid T_s \cup T_s &\ \  & \mathrm{(set\ terms)}\\
%T_i & ::= &  \min(S) \mid \max(S) & \ \ & \mathrm{(integer\ terms)}
%%t_i & ::= & c \mid \inf(S) \mid \sup(S) \mid ct_i \mid t_i + t_i
%\end{array}
%\]

%Wlog we assume that $\varphi_R(S,S')$ is satisfiable. 
Recall that, owing to the simplicity of $\dbs$, in $\varphi_R(S,S')$, the integer terms $t_i$ are $\min(S)$, $\max(S)$, $\min(S')$, or $\max(S')$ whereas the bounded-set terms $t_s$ are $\emptyset$, $\{\min(S)\}$, $\{\min(S')\}$, $\{\max(S)\}$, or $\{\max(S')\}$. It turns out the encoding is  rather technical, but not difficult. 
%To examplify, we assume that $\varphi_R(S,S')$ contains only set equalities (but not set inequalities), that is, formulae of the form $S  = S' \cup t_s$ or $S' = S \cup t_s$. 

For easy reference, we write $\varphi_R(S, S') = \varphi_{R,1} \wedge \varphi_{R,2}$, where $\varphi_{R,1}$ is an equality of set terms (i.e, they are of the form $S = S' \cup \{t_s\}$ or $S' = S \cup \{t_s\}$), and $\varphi_{R,2}$ is a conjunction of integer terms (i.e, it is a conjunction of the formulae $ t_i \ \le\ t_i + c$). 
%Moreover, $\lfloor\varphi_{R,2}\rfloor$ is part of $\varphi_{R,2}$ with $\max(S)/\min(S)$ or $\max(S')/\min(S')$ only. %by removing all conjuncts involving both $\max(S)$ and $S'$.

For technical convenience, we introduce a concept of saturation.

\begin{definition}[Saturated $\dbs$ formulae]
Let $\varphi_R(S, S') = \varphi_{R,1} \wedge \varphi_{R,2}$ be a $\dbs$ formula with $\varphi_{R,1} = S = S' \cup \{t_s\}$. 
%Since $\min(S'), \max(S') \in S'$, w.l.o.g., we assume that $t_s \subseteq \{\min(S), \max(S)\}$. 
Then $\varphi_R(S, S')$ is saturated if the following conditions hold.
\begin{itemize}
\item If $\min(S)$ or $\max(S)$ (resp. $\min(S')$ or $\max(S')$) occurs in $\varphi_R$, then $\varphi_{R,2}$ contains the conjunct $\min(S) \le \max(S)$ (resp. $\min(S') \le \max(S')$),
%
\item if  $\min(S)$ or $\max(S)$, as well as $\min(S')$ or $\max(S')$, occurs in $\varphi_R$, then $\varphi_{R,2}$ contains the conjuncts $\min(S) \le \min(S')$ and $\max(S') \le \max(S)$,
%
\item if $T_1 \le T_2 + c_1$ and $T_2 \le T_3 + c_2$ occur in $\varphi_{R,2}$, moreover, there is no conjunct $T_1 \le T_3 + c'$ in $\varphi_{R,2}$ such that $c' < c_1 + c_2$, then  $\varphi_{R,2}$ contains the conjunct $T_1 \le T_3 + c_1 + c_2$.
\end{itemize}
If $\varphi_R(S,S')$ is not saturated, then we can saturate $\varphi_R(S,S')$ by adding the missing conjuncts for the first two conditions above, then saturating the resulted difference-bound integer constraint $\varphi_{R,2}$ (reference here). 
\end{definition}

\tl{do we really need this saturation?}\zhilin{yes, put an example below to illustrate.}



\begin{example}
Let $\varphi_R(S,S') = \varphi_{R,1} \wedge \varphi_{R,2}$, where $\varphi_{R,1} = S = S' \cup \{\min(S)\}$ and $\varphi_{R,2}= \min(S') = \min(S)+1$. Then we saturate $\varphi_R(S,S')$ as follows: 
\begin{enumerate}
\item Since $\min(S)$ and $\min(S')$ occur in $\varphi_R$, let 
$$\varphi_{R,2} := \min(S') = \min(S)+1 \wedge \min(S) \le \max(S) \wedge \min(S') \le \max(S').$$
%
\item Because $\min(S)$ and $\min(S')$ occur in $\varphi_R(S,S')$, let 
$$
\begin{array}{r c l}
\varphi_{R,2} &:= & \min(S') = \min(S)+1 \wedge \min(S) \le \max(S) \wedge \min(S') \le \max(S') \wedge \\
& & \min(S) \le \min(S') \wedge \max(S') \le \max(S).
\end{array}
$$
See Figure~\ref{fig-varphi-r-2}(a) for the graphical illustration, where an edge from $\min(S')$ to $\min(S)$ of the weight $+1$, for instance, denotes the inequality $\min(S') \le \min(S)+1$. 
%
\item Saturate $\varphi_{R,2}$ by utilising the transitivity of $\le$, resulting into the following formula (see Figure~\ref{fig-varphi-r-2}(b)),
$$
\begin{array}{r c l}
\varphi_{R,2} &:= &   \min(S) \le \max(S)-1 \wedge \min(S) \le \max(S')-1 \wedge \\
& &  \min(S') = \min(S)+1 \wedge  \min(S') \le \max(S')   \wedge  \\
& & \min(S') \le \max(S) \wedge \max(S') \le \max(S).
\end{array}
$$
\end{enumerate}
\end{example}

\begin{figure}[htbp]
\begin{center}
\includegraphics{varphi-r-2.pdf}
\caption{$\varphi_{R,2}$ and its saturation.}
\label{fig-varphi-r-2}
\end{center}
\end{figure}




We proceed by a case-by-case analysis of $\varphi_{R,1}$. By symmetry, we focus on %illustrate the arguments by assuming that $\varphi_{R,1}$ is of the form 
the case $S = S' \cup \{t_s\}$.


\smallskip

\noindent {\bf \underline{Case I: $\varphi_{R,1} \equiv S = S'$}}. $\TC[\varphi_R](S, S') = \varphi_R(S, S')$.

\smallskip

\noindent {\bf \underline{Case II: $\varphi_{R,1} \equiv S = S' \cup \{\min(S)\}$}}. Then we have $\varphi_{R} \models S' \subseteq S$, and thus $\varphi_R \models \min(S) \le \min(S') \wedge \sup(S') \le \sup(S)$. If, furthermore, $\varphi_R \models \min(S) = \min(S')$, we have $\varphi_R \models S = S'$ and $\TC[\varphi_R](S, S') = \varphi_R(S, S')$. We then assume that $\varphi_R \not \models \min(S) = \min(S')$.
 
 


\smallskip

%Let $c_1$ be the maximum number $c$ such that $\min(S) \le \min(S') - c$ for $c \ge 0$ is a conjunct of $\varphi_{R,2}$. In addition, if $\varphi_{R,2}$ contains a conjunct $\min(S') \le \min(S) + c$ for $c > 0$, then let $c_2$ be the minimum such a number $c$, otherwise, let $c_2 = +\infty$. 

\noindent {\bf Subcase I(i): $\varphi_{R,2}$ contains a conjunct of the form $ \inf(S')  \le \inf(S) + c$.}

\smallskip

Clearly $c> 0$ and $\inf(S') \neq +\infty$, so $S' \neq \emptyset$. Let $c_1:=\max\{c\geq 0\mid \varphi_{R,2} 
%\mbox{ contains a conjunct }
\models\inf(S) \le \inf(S') - c\}$ 
%be the maximum number $c \ge 0$ such that $\varphi_{R,2}$ contains a conjunct $\inf(S) \le \inf(S') - c$. In addition, let 
and $c_2:=\min\{c\mid \varphi_{R,2} \models \inf(S') \le \inf(S) + c\}$.  Note that, according to the assumption of the case, $c_1, c_2\geq 0$. 
%
%$c_2$ be the minimum number $c > 0$ such that $\varphi_{R,2}$ contains a conjunct $\inf(S') \le \inf(S) + c$.  
%
We then have $\TC[\varphi_R](S, S')$ is 
%
$$(S = S') \vee  
\left(
\begin{array}{l}
S' \subseteq S \wedge S \neq \emptyset \wedge S' \neq \emptyset \wedge\\
(S \setminus S' \neq \emptyset \rightarrow \sup(S \setminus S') + c_1 \le \inf(S') \le \sup(S \setminus S') + c_2)\ \wedge \\
%\wedge (\forall y \in S \setminus S'.\ y < \inf(S')) \wedge \\
 \forall y, z \in S \setminus S'.\ (y < z \wedge (\forall z' \in S \setminus S'.\ (z' \le y \vee z \le z'))) \rightarrow y+ c_1 \le z \le y + c_2 \\
  \wedge \lfloor\varphi_{R,2}\rfloor
\end{array}
\right),
$$ 
%where 
%$\varphi'_{R,2}$ is the formula obtained from $\varphi_{R,2}$ by removing all conjuncts involving both $S$ and $S'$. 

\begin{example} Let $\varphi_{\plseg}(S, S') = S= S' \cup \{\inf(S)\} \wedge \inf(S') = \inf(S)+1$. This falls into subcase I(i) and we have $c_1=c_2=1$. One can easily obtain that 
	\[
	\begin{array}{l}
	\TC[\varphi_\plseg](S, S') = (S = S') \vee \\
	\hspace{1cm} (\emptyset \subset S' \wedge S' \subset S \wedge  \forall x.\ (x \in S \setminus S' \leftrightarrow \inf(S) \le x \le \inf(S') - 1)).
	\end{array}
	\]
\end{example}


\smallskip

\noindent {\bf Subcase I(ii): $\varphi_{R,2}$ does \emph{not} contain any conjunct of the form $ \inf(S')  \le \inf(S) + c$.}

\smallskip

%Then it is possible that $\inf(S') = +\infty$ and $S' = \emptyset$.

%Let $c_1$ be the maximum number $c \ge 0$ such that $\varphi_{R,2}$ contains a conjunct $\inf(S) \le \inf(S') - c$. 

$c_1:=\max\{c\geq 0\mid \varphi_{R,2} 
%\mbox{ contains a conjunct }
\models\inf(S) \le \inf(S') - c\}$. Then $\TC[\varphi_R](S, S')$ is 
%
$$(S = S') \vee  
\left(
\begin{array}{l}
S' \subseteq S \wedge S \neq \emptyset \wedge 
((S \setminus S' \neq \emptyset  \wedge S' \neq \emptyset) \rightarrow \sup(S \setminus S') \le \inf(S') - c_1) \ \wedge \\
%\wedge (\forall y \in S \setminus S'.\ y < \inf(S')) \wedge \\
 \forall y, z \in S \setminus S'.\ (y < z \wedge (\forall z' \in S \setminus S'.\ (z' \le y \vee z \le z'))) \rightarrow y \le z - c_1 \\
  \wedge \lfloor\varphi_{R,2}\rfloor
\end{array}
\right),
$$ 
%where 
%$\varphi'_{R,2}$ is the formula obtained from $\varphi_{R,2}$ by removing every conjunct that involves both $S$ and $S'$. 

%=============================================case II ==========================================
\smallskip

\noindent {\bf \underline{Case II: $\varphi_{R,1} \equiv S = S' \cup \{\max(S)\}$}}.

This is similar to (actually symmetrical to) Case I, the details are given in Appendix~\ref{app:subcaseII}.
%\smallskip
%
%Then we have $\varphi_{R} \models S' \subseteq S$. Therefore, $\varphi_R \models \inf(S) \le \inf(S') \wedge \sup(S') \le \sup(S)$. 
%
%If $\varphi_R \models \sup(S) = \sup(S')$, then we have $\varphi_R \models S = S'$. Therefore, we have $TC[\varphi_R](S, S') = \varphi_R(S, S')$. 
%
%In the following, let us assume that $\varphi_R \not \models \sup(S) = \sup(S')$.
%
%We assume that $\varphi_R$ is \emph{saturated}, in the following sense,
%\begin{itemize}
%%
%\item $\varphi_{R,2}$ contains the conjunct $\inf(S) \le \sup(S)$, since $\varphi_R \models S \neq \emptyset$,
%%
%\item if $\varphi_R \models S' \neq \emptyset$, then $\varphi_{R,2}$ contains the conjunct $\inf(S') \le \sup(S')$,
%%
%\item $\varphi_{R,2}$ contains the conjuncts $\inf(S) \le \inf(S')$ and $\sup(S') \le \sup(S)$,
%%
%%\item if $\varphi_{R,1}$ contains a conjunct $S \subseteq S'$ (resp. $S' \subseteq S$), then $\inf(S') \le \inf(S)$ and $\sup(S) \le \sup(S')$ (resp. $\inf(S) \le \inf(S')$ and $\sup(S') \le \sup(S)$) are the conjuncts of $\varphi_{R,2}$,
%%
%\item if $\varphi_{R,2}$ contains $t_1 \le t_2 + c_1$ and $t_2 \le t_3 + c_2$, moreover, there is no $t_1 \le t_3 + c'$ such that $c' < c_1 + c_2$, then  add $t_1 \le t_2 + c_1 + c_2$ as a conjunct of $\varphi_{R,2}$.
%\end{itemize}
%
%
%\noindent {\bf Subcase II(i): $\varphi_{R,2}$ contains a conjunct of the form $ \sup(S)  \le \sup(S') + c$ for some $c> 0$.}
%
%\smallskip
%
%Then we know that $\sup(S') \neq +\infty$, so $S' \neq \emptyset$. 
%
%Let $c_1$ be the maximum number $c \ge 0$ such that $\varphi_{R,2}$ contains a conjunct $\sup(S') \le \sup(S) - c$. In addition, let $c_2$ be the minimum number $c > 0$ such that $\varphi_{R,2}$ contains a conjunct $\sup(S) \le \sup(S') + c$.  Evidently, $c_1 \le c_2$, since otherwise $\varphi_{R,2}$ is unsatisfiable.
%
%Then $TC[\varphi_R](S, S')$ is 
%%
%$$(S = S') \vee  
%\left(
%\begin{array}{l}
%S' \subseteq S \wedge S \neq \emptyset \wedge S' \neq \emptyset \wedge \\
%(S \setminus S' \neq \emptyset \rightarrow \inf(S \setminus S') - c_2 \le \sup(S') \le \inf(S \setminus S') - c_1)\ \wedge \\
%%\wedge (\forall y \in S \setminus S'.\ y < \inf(S')) \wedge \\
% \forall y, z \in S \setminus S'.\ (y < z \wedge (\forall z' \in S \setminus S'.\ (z' \le y \vee z \le z'))) \rightarrow z - c_2 \le y \le z - c_1 \\
%  \wedge \varphi'_{R,2}
%\end{array}
%\right),
%$$ 
%where 
%$\varphi'_{R,2}$ is the formula obtained from $\varphi_{R,2}$ by removing every conjunct that involves both $S$ and $S'$. 
%
%\smallskip
%
%\noindent {\bf Subcase II(ii): $\varphi_{R,2}$ does not contain a conjunct of the form $ \sup(S)  \le \sup(S') + c$ for some $c> 0$.}
%
%\smallskip
%
%Then it is possible that $\sup(S') = -\infty$ and $S' = \emptyset$.
%
%Let $c_1$ be the maximum number $c \ge 0$ such that $\varphi_{R,2}$ contains a conjunct $\sup(S') \le \sup(S) - c$. 
%
%Then $TC[\varphi_R](S, S')$ is 
%%
%$$(S = S') \vee  
%\left(
%\begin{array}{l}
%S' \subseteq S \wedge S \neq \emptyset \wedge 
%((S \setminus S' \neq \emptyset  \wedge S' \neq \emptyset) \rightarrow \sup(S') \le \inf(S \setminus S') - c_1) \ \wedge \\
%%\wedge (\forall y \in S \setminus S'.\ y < \inf(S')) \wedge \\
% \forall y, z \in S \setminus S'.\ (y < z \wedge (\forall z' \in S \setminus S'.\ (z' \le y \vee z \le z'))) \rightarrow y \le z - c_1 \\
%  \wedge \varphi'_{R,2}
%\end{array}
%\right),
%$$ 
%where 
%$\varphi'_{R,2}$ is the formula obtained from $\varphi_{R,2}$ by removing every conjunct that involves both $S$ and $S'$. 

%============================================= case III ========================================

\smallskip

\noindent {\bf \underline{Case III: $\varphi_{R,1} \equiv S = S' \cup \{\min(S), \max(S)\}$}}.

\begin{example}
\[
\varphi(S, S') = S = S' \cup \{\inf(S), \sup(S)\} \wedge \inf(S)+2 = \inf(S') \wedge \sup(S')+2 = \sup(S).
\]
Then 
\[
\TC[\varphi](S, S') = (S = S') \vee
\left(\begin{array}{l}
\wedge S' \subseteq S \wedge S' \neq \emptyset \wedge S \setminus S' = S_1 \cup S_2\ \wedge \\
S_1 \cap S_2 = \emptyset \wedge S_1 \neq \emptyset \wedge S_2 \neq \emptyset\ \wedge \\
 \sup(S_1) + 2 = \inf(S') \wedge \sup(S') + 2 = \inf(S_2)\ \wedge \\
 \forall x.\  x \in S_1 \leftrightarrow (\inf(S_1) \le x \le \sup(S_1) \wedge \inf(S') - x \equiv 0 \bmod 2)\ \wedge \\
 \forall x.\  x \in S_2 \leftrightarrow (\inf(S_2) \le x  \le \sup(S_2) \wedge x- \sup(S') \equiv 0 \bmod 2) \wedge \\
  \sup(S_1)- \inf(S_1) = \sup(S_2) - \inf(S_2)  
\end{array}
\right).
\]

%The sub-formula $ \inf(S_1) + 2 z = \sup(S_1) \wedge \inf(S_2) + 2 z = \sup(S_2)$ in $TC[\Delta](S, S')$ goes beyond $\dbs$.
 
\end{example}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\hide{
\zhilin{The following texts should be cleaned. Let us focus on the $S  = S' \cup t_s$ above first.}

\smallskip

\noindent {\bf $S \subseteq S' \cup t_s$}.
\begin{itemize}
\item $t_s = \emptyset$: In this case, we have $S \subseteq S'$. Therefore, $\inf(S') \le \inf(S) $ and $\sup(S) \le \sup(S')$.  Then $TC[\varphi_R](S, S') = S \subseteq S' \wedge \psi_1 \wedge \psi_2 \wedge \varphi'_R(S,S')$, where $\varphi'_R(S,S')$ is obtained from $\varphi'_R(S,S')$ by removing $S \subseteq S'$ and the atomic formulae of the form $\inf(S') + c\ o\ \inf(S)$ or $\sup(S') + c\ o\ \sup(S)$,
\begin{itemize}
\item define $\psi_1$ as follows:
\begin{itemize}
\item if $\inf(S) \le \inf(S')$ and $\inf(S') \le \inf(S)$ are conjuncts of $\varphi_R(S,S')$, then let $\psi_1 = \inf(S) = \inf(S')$, 
%
\item if $\inf(S') \le \inf(S) - c$ and $\inf(S) \le \inf(S') + c$ are conjuncts of $\varphi_R(S,S')$ for some $c>0$, then let $\psi_1 = \inf(S) - \inf(S') \equiv 0 \bmod c$,
%
\item if $\inf(S') \le \inf(S) - c$  is a conjunct of $\varphi_R(S,S')$ for some $c>0$, then let $\psi_1 = c \le \inf(S) - \inf(S')$,
%
\item otherwise, $\psi_1 = \ltrue$,
\end{itemize}
%
\item define $\psi_2$ as follows: 
\begin{itemize}
\item if $\sup(S) \le \sup(S')$ and $\sup(S') \le \sup(S)$ are conjuncts of $\varphi_R(S,S')$, then let $\psi_2 = \sup(S) = \sup(S')$, 
%
\item if $\sup(S) + c \le \sup(S')$ and $\sup(S') \le \sup(S) + c$ are conjuncts of $\varphi_R(S,S')$ for some $c>0$, then let $\psi_2 = \sup(S') - \sup(S) \equiv 0 \bmod c$,
%
\item if $\sup(S) + c \le \sup(S')$ is a conjunct of $\varphi_R(S,S')$ for some $c > 0$, then let $\psi_2 = c \le \sup(S') - \sup(S)$,
%
\item otherwise, $\psi_2 = \ltrue$.
\end{itemize}
\end{itemize}
%
\item $t_s = \{\inf(S)\}$: 
\begin{itemize}
\item if $\inf(S') \le \inf(S)+c$ and $\inf(S) \le \inf(S')-c$ for some $c < 0$ are conjuncts of $\varphi_{R,2}$, then $TC[\varphi_R](S,S')=S \setminus{\inf(S)} \subseteq S' \wedge \inf(S') \le \inf(S)+ c \wedge \inf(S)-\inf(S') \equiv 0 \bmod (-c) \wedge \psi \wedge \varphi'_{R,2}$, where $\varphi'_{R,2}$ is obtained from $\varphi_{R,2}$ by removing all the atomic formulae involving both $S$ and $S'$, and $\psi$ is defined as follows,
\begin{itemize}
\item if $ \sup(S) \le \sup(S') + c'$ and $ \sup(S') \le \sup(S) - c'$ for some $c'<0$ are conjuncts of $\varphi_{R,2}$, then $\psi =  \sup(S) \le \sup(S') + c' \wedge \sup(S') -  \sup(S)  \equiv 0 \bmod (-c')$,
%
\item otherwise, if $\sup(S) \le \sup(S')$ and $\sup(S') \le \sup(S)$ are the conjuncts of $\varphi_{R,2}$, then $\psi = \sup(S) \le \sup(S') \wedge \sup(S') \le \sup(S)$,
%
\item otherwise, if $\sup(S') \le \sup(S)+c'$ and $\sup(S) \le \sup(S') - c'$ for some $c'<0$ are conjuncts of $\varphi_{R,2}$, then $\psi = S = \{\inf(S)\}  \wedge  \sup(S') \le \sup(S)+c' \wedge \sup(S) - \sup(S') \equiv 0 \bmod (-c')$,
%
\item otherwise, if $\sup(S') \le \sup(S)+c'$  for some $c'<0$ is a conjunct of $\varphi_{R,2}$, then $\psi = S = \{\inf(S)\}  \wedge \sup(S') \le \sup(S)+c'$,
\end{itemize}
%
\item if $\inf(S) \le \inf(S')$ and $\inf(S') \le \inf(S)$ are conjuncts of $\varphi_{R,2}$, then $TC[\varphi_R](S,S')=S \setminus{\inf(S)} \subseteq S' \wedge \inf(S) \le \inf(S') \wedge \inf(S') \le \inf(S)$,
%
\item otherwise, 
if $\inf(S') \le \inf(S)  + c$ for some $c \le 0$ is a conjunct of $\varphi_{R,2}$, then $TC[\varphi_R](S,S')=S \setminus{\inf(S)} \subseteq S'$,
%
\end{itemize}

Then $TC[\varphi_R](S,S') =(S = S') \vee (S \neq \emptyset \wedge \psi_1 \wedge \psi_2 \wedge \varphi'_{R,2}) \vee (\exists S_1, S_2.\ S = S_1 \cup S_2 \wedge S_1 \cap S_2 = \emptyset \wedge S_1 \neq \emptyset \wedge S_2 \neq \emptyset \wedge \sup(S_1) < \inf(S_2) \wedge S_2 \subseteq S' \wedge \psi_3 \wedge \psi_4 \wedge \varphi'_{R,2})$, where
\begin{itemize}
\item $\psi_1$ is defined as follows,
\begin{itemize}
\item if $\inf(S) \le \inf(S')$ and $\inf(S') \le \inf(S)$ are conjuncts of $\varphi_{R,2}$, then $\psi_1= \inf(S) \le \inf(S') \wedge \inf(S') \le \inf(S)$,
%
\item if $\inf(S) \le \inf(S') + c$ for some $c < 0$ is a conjunct of $\varphi_{R,2}$, then $\psi_1 =\sup(S) \le \inf(S')+c \wedge \forall x, y.\ (x,y \in S \wedge x < y ) \rightarrow (x \le y + c)$,
%
\item otherwise, $\inf(S') \le \inf(S)  + c$ for some $c \le 0$ is a conjunct of $\varphi_{R,2}$, then $\psi_1 = \inf(S') \le \inf(S) + c$,
\end{itemize} 
%
\item $\psi_2$ is defined as follows,
\begin{itemize}
\item if $\sup(S) \le \sup(S')$ and $\sup(S') \le \sup(S)$ are conjuncts of $\varphi_{R,2}$, then $\psi_2=(S_2 = \emptyset \wedge \sup(S_1) \le \sup(S') \wedge \sup(S') \le \sup(S_1)) \vee (S_2 \neq \emptyset \wedge \sup(S_2) \le \sup(S') \wedge \sup(S') \le \sup(S_2))$,
%
\item if $\sup(S) \le \sup(S') + c$ for some $c < 0$ is a conjunct of $\varphi_{R,2}$, then $\psi_2 =(S_2 = \emptyset 
\wedge \sup(S_1) \le \sup(S') + c) \vee (S_2 \neq \emptyset \wedge \sup(S_2) \le \sup(S') + c)$,
%
\item otherwise, $\inf(S') \le \inf(S)  + c$ for some $c \le 0$ is a conjunct of $\varphi_{R,2}$, then $\psi_1 = \inf(S') \le \inf(S) + c$,
\end{itemize} 
%
\item $\psi_3$ is defined as follows,
\begin{itemize}
\item if $\inf(S) \le \inf(S')$ and $\inf(S') \le \inf(S)$ are conjuncts of $\varphi_{R,2}$, then $\psi_1= \inf(S_1) \le \inf(S') \wedge \inf(S') \le \inf(S_1)$,
%
\item if $\inf(S) \le \inf(S') + c$ for some $c < 0$ is a conjunct of $\varphi_{R,2}$, then $\psi_1 =\inf(S_1) \le \inf(S')+c \wedge \forall x, y.\ (x,y \in S_1 \wedge x < y ) \rightarrow (x \le y + c)$,
%
\item otherwise, $\inf(S') \le \inf(S)  + c$ for some $c \le 0$ is a conjunct of $\varphi_{R,2}$, then $\psi_1 = \inf(S') \le \inf(S) + c$,
\end{itemize} 
%
\item $\psi_4$ is defined as follows,
\begin{itemize}
\item if $\sup(S) \le \sup(S')$ and $\sup(S') \le \sup(S)$ are conjuncts of $\varphi_{R,2}$, then $\psi_2=(S_2 = \emptyset \wedge \sup(S_1) \le \sup(S') \wedge \sup(S') \le \sup(S_1)) \vee (S_2 \neq \emptyset \wedge \sup(S_2) \le \sup(S') \wedge \sup(S') \le \sup(S_2))$,
%
\item if $\sup(S) \le \sup(S') + c$ for some $c < 0$ is a conjunct of $\varphi_{R,2}$, then $\psi_2 =(S_2 = \emptyset 
\wedge \sup(S_1) \le \sup(S') + c) \vee (S_2 \neq \emptyset \wedge \sup(S_2) \le \sup(S') + c)$,
%
\item otherwise, $\inf(S') \le \inf(S)  + c$ for some $c \le 0$ is a conjunct of $\varphi_{R,2}$, then $\psi_1 = \inf(S') \le \inf(S) + c$,
\end{itemize} 
%
\item $\varphi'_{R,2}$ is obtained from $\varphi_{R,2}$ by removing all the atomic formulae that contains both $S$ and $S'$,
\end{itemize}
%
\item $t_s = \{\sup(S)\}$: 
%
\item $t_s = \{\inf(S), \sup(S)\}$: 
\end{itemize}

\smallskip

\noindent {\bf $S \supseteq S' \cup t_s$}.

\smallskip

\noindent {\bf $S \subset S' \cup t_s$}.

\smallskip

\noindent {\bf $S \supset S' \cup t_s$}.
}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\smallskip

\paragraph{General cases.} For the general case, we may assume that in $\varphi_R(\vec{S}; \vec{S'})$, the parameters in different positions are \emph{independent} in every atomic set formulae. For instance, in $\varphi_R(S_1, S_2; S'_1, S'_2)$, for each atomic formula of the form $S = S' \cup t_s$, either all the variables in $S = S' \cup t_s$ are from $\{S_1, S'_1\}$, or all of them are from $\{S_2, S'_2\}$.

Let us start with an example.

\zhilin{The following example shows that the satisfiability of $\varphi_R(\vec{S}; \vec{S'})$ with multiple source parameters is challenging to solve.}

$\varphi_R(S_1, S_2; S'_1, S'_2)\equiv  S_1 = S'_1 \cup \{\inf(S_1)\} \wedge S_2 = S'_2 \cup \{\inf(S_2)\} \wedge \inf(S_1) +2 = \inf(S'_1) \wedge \inf(S_2) +2 = \inf(S'_2)$.

Then $TC[\varphi_R](S_1, S_2; S'_1, S'_2)$ is 
$$
\begin{array}{l}
(S_1=S'_1 \wedge S_2 = S'_2)\ \vee \\
\left(
\begin{array}{l}
S'_1 \subset S_1 \wedge S'_2 \subset S_2 \wedge S_1 \neq \emptyset \wedge S_2 \neq \emptyset \wedge S'_1 \neq \emptyset \wedge S'_2 \neq \emptyset \\
\sup(S_1 \setminus S'_1) + 2 = \inf(S'_1) \wedge \sup(S_2 \setminus S'_2) + 2 = \inf(S'_2) \wedge\\
 \forall y, z \in S_1 \setminus S'_1.\ (y < z \wedge (\forall z' \in S_1 \setminus S'_1.\ (z' \le y \vee z \le z'))) \rightarrow y+2 = z\ \wedge \\
  \forall y, z \in S_2 \setminus S'_2.\ (y < z \wedge (\forall z' \in S_2 \setminus S'_2.\ (z' \le y \vee z \le z'))) \rightarrow y+2 = z \\
  \wedge \exists x.\ (\inf(S_1) + 2 x = \inf(S'_1) \wedge \inf(S_2) + 2 x= \inf(S'_2))
\end{array}
\right).
\end{array}
$$

The formula $\inf(S_1) + 2 x = \inf(S'_1) \wedge \inf(S_2) + 2 x= \inf(S'_2)$ also goes beyond $\dbs$.

%====================================================== end of section=======================================
